Personalized Online Machine Learning

In this work, we introduce the Personalized Online Super Learner (POSL) -- an online ensembling algorithm for streaming data whose optimization procedure accommodates varying degrees of personalization. Namely, POSL optimizes predictions with respect to baseline covariates, so personalization can vary from completely individualized (i.e., optimization with respect to baseline covariate subject ID) to many individuals (i.e., optimization with respect to common baseline covariates). As an online algorithm, POSL learns in real-time. POSL can leverage a diversity of candidate algorithms, including online algorithms with different training and update times, fixed algorithms that are never updated during the procedure, pooled algorithms that learn from many individuals' time-series, and individualized algorithms that learn from within a single time-series. POSL's ensembling of this hybrid of base learning strategies depends on the amount of data collected, the stationarity of the time-series, and the mutual characteristics of a group of time-series. In essence, POSL decides whether to learn across samples, through time, or both, based on the underlying (unknown) structure in the data. For a wide range of simulations that reflect realistic forecasting scenarios, and in a medical data application, we examine the performance of POSL relative to other current ensembling and online learning methods. We show that POSL is able to provide reliable predictions for time-series data and adjust to changing data-generating environments. We further cultivate POSL's practicality by extending it to settings where time-series enter/exit dynamically over chronological time.

==> Personalized Online Ensemble Machine Learning/_glossary.tex <==
\newglossaryentry{gls_tau} {
  name={\ensuremath{\tau}},
  text={\ensuremath{\tau}},
  description={total number of chronological time points; index for time is $t$}
} 

\newglossaryentry{gls_n} {
  name={\ensuremath{n}},
  text={\ensuremath{n}},
  description={total number of sampled subjects; index for samples is $i$}
}

\newglossaryentry{gls_Yt} {
  name={\ensuremath{Y_i(t)}},
  text={\ensuremath{Y_i(t)}},
  description={time $t$-specific response variable for sample $i$}
}

\newglossaryentry{gls_Wt} {
  name={\ensuremath{W_i(t)}},
  text={\ensuremath{W_i(t)}},
  description={time $t$-specific time-varying covariates for sample $i$}
}

\newglossaryentry{gls_Ot} {
  name={\ensuremath{O_i(t)}},
  text={\ensuremath{O_i(t)}},
  description={time $t$-specific p-dimensional random variable for sample $i$ where $O_i(t) = (W_i(t), Y_i(t))$}
}

\newglossaryentry{gls_X} {
  name={\ensuremath{X_i}},
  text={\ensuremath{X_i}},
  description={vector of baseline covariates for sample $i$}
}

\newglossaryentry{gls_On} {
  name={\ensuremath{O^n}},
  text={\ensuremath{O^n}},
  description={collection of $n$ time-series}
}

\newglossaryentry{gls_P0} {
  name={\ensuremath{P_0^n}},
  text={\ensuremath{P_0^n}},
  description={true probability distribution of $(X^n,O^n)$}
}

\newglossaryentry{gls_Px} {
  name={\ensuremath{P_{0,O_i|X_i}}},
  text={\ensuremath{P_{0,O_i|X_i}}},
  description={true conditional distribution of $O_i$ given $X_i$ (short notation: $P_{0,X_i}$)}
}

\newglossaryentry{gls_M} {
  name={\ensuremath{\mathcal{M}}},
  text={\ensuremath{\mathcal{M}}},
  description={statistical model, such that the true data-generating distribution is an element of it ($P_0^n \in \mathcal{M}$)}
}

\newglossaryentry{gls_Obar} {
  name={\ensuremath{\overline{O}_i(t-1)}},
  text={\ensuremath{\overline{O}_i(t-1)}},
  description={time $t$-specific history of the time-series for sample $i$, where $\overline{O}_i(t-1) = (O_i(1),  \ldots, O_i(t-1))$}
}

\newglossaryentry{gls_Onbar} {
  name={\ensuremath{\overline{O}^n(t-1)}},
  text={\ensuremath{\overline{O}^n(t-1)}},
  description={time $t$-specific history of $n$ time-series, where $\overline{O}^n(t-1) = \{\overline{O}_1(t-1), \ldots,  \overline{O}_n(t-1)\}$}
}

\newglossaryentry{gls_Pcommon} {
  name={\ensuremath{P_{0,O_i}}},
  text={\ensuremath{P_{0,O_i}}},
  description={true common conditional distribution of $O_i$ given $Z_{i}(t-1)$ and $X_i$}
}

\newglossaryentry{gls_Z} {
  name={\ensuremath{Z_i(t-1)}},
  text={\ensuremath{Z_i(t-1)}},
  description={time $t$-specific fixed dimensional summary measure for sample $i$}
}

\newglossaryentry{gls_Psi} {
  name={\ensuremath{\Psi}},
  text={\ensuremath{\Psi}},
  description={parameter mapping, a function from an element of the statistical model $\mathcal{M}$ ($P$) into the parameter space, $\pmb{\Psi}$}
  }
  
\newglossaryentry{gls_psi} {
  name={\ensuremath{\psi}},
  text={\ensuremath{\psi}},
  description={parameter mapping evaluated at a probability distribution in the statistical model, where $\psi \coloneqq \Psi(P)$ for $P \in \mathcal{M}$}
  }
  
\newglossaryentry{gls_estimand} {
  name={\ensuremath{\Psi(P_0^n)(X_i,Z_i(t-1),t)}},
  text={\ensuremath{\Psi(P_0^n)(X_i,Z_i(t-1),t)}},
  description={prediction function evaluated at the truth for the $i^{\text{th}}$ subject and time $t$}
  }  
  
\newglossaryentry{gls_loss} {
  name={\ensuremath{L(\Psi(P))(X_i,Y_i(t),Z_i(t-1))}},
  text={\ensuremath{L(\Psi(P))(X_i,Y_i(t),Z_i(t-1))}},
  description={loss function corresponding to $\Psi(P)$ evaluated for sample $i$ at time $t$; equivalently, we write $L(\psi)(X_i,Y_i(t),Z_i(t-1))$ for $\psi \coloneqq \Psi(P)$}
  }
  
\newglossaryentry{gls_risk} {
  name={\ensuremath{R(P_{0}^n, \psi)}},
  text={\ensuremath{R(P_{0}^n, \psi)}},
  description={true risk of $\psi$, defined as the sum over time and samples of the expected value of the loss with respect to $P_{0}^n$; 
  $R(P_{0}^n, \psi) = \frac{1}{n} \sum_{i=1}^n  \sum_{t=1}^{\tau} E_{P_{0,O_i}} [L(\psi)(X_i,Y_i(t),Z_i(t-1)) | X_i, Z_i(t-1)]$}
  }   
  
\newglossaryentry{gls_psi_0} {
  name={\ensuremath{\psi_{0}}},
  text={\ensuremath{\psi_{0}}},
  description={predictive function corresponding to $\hat{\Psi}(P_{0}^n)$; minimizer over the true risk of all evaluated $\psi$ in the parameter space}
  }  
 
\newglossaryentry{gls_psi_0i} {
  name={\ensuremath{\psi_{0,i}}},
  text={\ensuremath{\psi_{0,i}}},
  description={minimizer over the true risk of all evaluated $\psi$ in the parameter space for sample $i$}
  }   
  
\newglossaryentry{gls_hatPsi} {
  name={\ensuremath{\hat{\Psi}}},
  text={\ensuremath{\hat{\Psi}}},
  description={estimator mapping, a function from the empirical distribution ($P_{n,t}$, at any $t$) to the parameter space, $\pmb{\Psi}$}
  }  

\newglossaryentry{gls_Pnt} {
  name={\ensuremath{P_{n,t}}},
  text={\ensuremath{P_{n,t}}},
  description={empirical distribution of $n$ time series collected until time $t$}
} 

\newglossaryentry{gls_psi_nt} {
  name={\ensuremath{\psi_{n,t}}},
  text={\ensuremath{\psi_{n,t}}},
  description={predictive function corresponding to $\hat{\Psi}(P_{n,t})$; $\hat{\Psi}(P_{n,t})$ maps $(X_i,Z_i(t-1),t)$ into a time- and subject-specific outcome, $Y_{i}(t)$}
  }
  
\newglossaryentry{gls_v} {
  name={\ensuremath{v}},
  text={\ensuremath{v}},
  description={fold number corresponding to the used cross-validation scheme}
  } 
  
\newglossaryentry{gls_C} {
  name={\ensuremath{C(i,s,\cdot)}},
  text={\ensuremath{C(i,s,\cdot)}},
  description={at minimum, time $s$- and unit $i$-specific record where $C(i,s,\cdot) = (X_i, Z_i(s-1), Y_i(s),\cdot)$}
} 
  
\newglossaryentry{gls_Bn} {
  name={\ensuremath{B_t^v(i,s,\cdot)}},
  text={\ensuremath{B_t^v(i,s,\cdot)}},
  description={$v$-fold assignment of unit $i$ at time point $s$ for split $B_t^v$ trained on data until time $t$. If dynamic enrollment setting, $B_t^v$ also includes starting time $E_i$}
} 

\newglossaryentry{gls_Pnt_0} {
  name={\ensuremath{P_{n,t}^0}},
  text={\ensuremath{P_{n,t}^0}},
  description={empirical distribution of the training sample until time $t$}
} 

\newglossaryentry{gls_Pnt_1} {
  name={\ensuremath{P_{n,t}^1}},
  text={\ensuremath{P_{n,t}^1}},
  description={empirical distribution of the validation sample until time $t$}
} 

\newglossaryentry{gls_nt_0} {
  name={\ensuremath{n_{t}^0}},
  text={\ensuremath{n_{t}^0}},
  description={number of observations in the training set for split $B_t$, over all folds $v$ until time $t$}
} 

\newglossaryentry{gls_nt_1} {
  name={\ensuremath{n_{t}^1}},
  text={\ensuremath{n_{t}^1}},
  description={number of observations in the validation set for split $B_t$, over all folds $v$ until time $t$}
}

\newglossaryentry{gls_Bt_0} {
  name={\ensuremath{\mathcal{B}_{t,v}^0}},
  text={\ensuremath{\mathcal{B}_{t,v}^0}},
  description={set of all $(i,s)$ indexes in the training set until time $t$ for fold $v$}
} 

\newglossaryentry{gls_Bt_1} {
  name={\ensuremath{\mathcal{B}_{t,v}^1}},
  text={\ensuremath{\mathcal{B}_{t,v}^1}},
  description={set of all $(i,s)$ indexes in the validation set until time $t$ for fold $v$}
} 

\newglossaryentry{gls_hatPsi_k} {
  name={\ensuremath{\hat{\Psi}_k}},
  text={\ensuremath{\hat{\Psi}_k}},
  description={estimator mapping for candidate algorithm $k$, a function from the empirical distribution ($P_{n,t}$, at any $t$) to the parameter space, $\pmb{\Psi}$}
  } 

\newglossaryentry{gls_psi_ntk_0} {
  name={\ensuremath{\psi_{n,t,k}^0}},
  text={\ensuremath{\psi_{n,t,k}^0}},
  description={predictive function corresponding to $\hat{\Psi}_k(P_{n,t}^0)$ based on the candidate algorithm $k$ and trained on the training set $P_{n,t}^0$ until time $t$}
  } 

\newglossaryentry{gls_risk_cv} {
  name={\ensuremath{R_{CV}(P_{n,t}^1, \hat{\Psi}_k(\cdot))}},
  text={\ensuremath{R_{CV}(P_{n,t}^1, \hat{\Psi}_k(\cdot))}},
  description={online cross-validated risk for candidate estimator $k$ defined as an empirical average of the loss with respect to $P_{n,t}^1$; in particular, we write $R_{CV}(P_{n,t}^1, \hat{\Psi}_k(\cdot)) = \sum_{j=1}^{t} \sum_{v=1}^V \sum_{(i,s) \in \mathcal{B}_{j,v}^1} L(\psi_{n,j,k}^0)(C(i,s))$}
  } 
  
\newglossaryentry{gls_risk_cv_true} {
  name={\ensuremath{R_{CV}(P_{0}^n, \hat{\Psi}_k(\cdot))}},
  text={\ensuremath{R_{CV}(P_{0}^n, \hat{\Psi}_k(\cdot))}},
  description={the true online cross-validated risk for candidate estimator $k$ defined as the expected value of the loss with respect to $P_{0}^n$; in particular, we write $R_{CV}(P_{0}^n, \hat{\Psi}_k(\cdot)) = \sum_{j=1}^{t} \sum_{v=1}^V \sum_{(i,s) \in \mathcal{B}_{j,v}^1} E_{P_{0,O_i}}[L(\psi_{n,j,k}^0)(C(i,s)) | X_i, Z_i(s-1)]$}
  }   
 
\newglossaryentry{gls_knt} {
  name={\ensuremath{k_{n,t}}},
  text={\ensuremath{k_{n,t}}},
  description={learner that minimizes the online cross-validated risk, the discrete online cross-validation selector}
}   
  
\newglossaryentry{gls_psi_discrete_0} {
  name={\ensuremath{\psi_{n, t, k_{n,t}}^0}},
  text={\ensuremath{\psi_{n, t, k_{n,t}}^0}},
  description={predictive function corresponding to $\hat{\Psi}_{k_{n,t}}(P_{n,t}^0)$, based on the discrete online cross-validation selector $k_{n,t}$ and trained on the training set $P_{n,t}^0$ until time $t$}
  } 

\newglossaryentry{gls_d0_i} {
  name={\ensuremath{d_{0,t}(\psi_{n,t,k,i}, \psi_{0,i})}},
  text={\ensuremath{d_{0,t}(\psi_{n,t,k,i}, \psi_{0,i})}},
  description={loss-based dissimilarity for sample $i$ between $k$ estimator $\hat{\Psi}_k$ evaluated until time $t$ and $\psi_{0,i}$ with respect to $P_{0,O_i}$}
} 

\newglossaryentry{gls_d0} {
  name={\ensuremath{d_{0,t}(\psi_{n,t,k}, \psi_0)}},
  text={\ensuremath{d_{0,t}(\psi_{n,t,k}, \psi_0)}},
  description={average of $i$-specific loss-based dissimilarities over all samples evaluated until time $t$}
}

\newglossaryentry{gls_knt_oracle} {
  name={\ensuremath{\overline{k}_{n,t}}},
  text={\ensuremath{\overline{k}_{n,t}}},
  description={oracle selector among discrete set of candidate estimators $\hat{\Psi}_k$ based on $P_{n,t}$.}
} 

\newglossaryentry{gls_hatPsi_alpha} {
  name={\ensuremath{\hat{\Psi}_{\alpha}}},
  text={\ensuremath{\hat{\Psi}_{\alpha}}},
  description={estimator mapping, a function from the empirical distribution ($P_{n,t}$, at any $t$) generating an ensemble of $K$ estimators $(\hat{\Psi}_1, \ldots, \hat{\Psi}_K)$ indexed by a vector of coefficients $\alpha$ $(\alpha_1, \ldots, \alpha_K)$}
  } 

\newglossaryentry{gls_psi_nta_0} {
  name={\ensuremath{\psi_{n,t,\alpha}^0}},
  text={\ensuremath{\psi_{n,t,\alpha}^0}},
  description={predictive function corresponding to $\hat{\Psi}_{\alpha}(P_{n,t}^0)$ based on the ensemble of $K$ candidate estimators with weights $\alpha$, trained on the training set $P_{n,t}^0$ until time $t$}
  } 
  
\newglossaryentry{gls_alpha} {
  name={\ensuremath{\alpha_{n,t}}},
  text={\ensuremath{\alpha_{n,t}}},
  description={weight for the ensemble of candidate estimators $\hat{\Psi}_k$ based on $P_{n,t}$ that minimizes the online cross-validated risk} 
} 

\newglossaryentry{gls_alpha_oracle} {
  name={\ensuremath{\overline{\alpha}_{n,t}}},
  text={\ensuremath{\overline{\alpha}_{n,t}}},
  description={oracle selector among weights of the ensemble of candidate estimators $\hat{\Psi}_k$ based on $P_{n,t}$}
} 

%Is it used?
\newglossaryentry{gls_psi_ntk} {
  name={\ensuremath{\psi_{n,t,k}}},
  text={\ensuremath{\psi_{n,t,k}}},
  description={predictive function corresponding to $\hat{\Psi}_k(P_{n,t})$ based on the candidate algorithm $k$}
  } 
 
%Dynamic defs
\newglossaryentry{gls_E} {
  name={\ensuremath{E_i}},
  text={\ensuremath{E_i}},
  description={chronological entry time for time-series $i$. We assume a natural ordering for all $E_i$, with $0 \leq E_1 \leq \ldots \leq E_n$ even if multiple samples enroll around the same time}
}

\newglossaryentry{gls_Mi} {
  name={\ensuremath{M_i}},
  text={\ensuremath{M_i}},
  description={length of the time-series $i$ from the start of follow-up to the last collected time point}
}

\newglossaryentry{gls_T} {
  name={\ensuremath{T_i}},
  text={\ensuremath{T_i}},
  description={chronological exit time for time-series $i$}
}

\newglossaryentry{gls_hi} {
  name={\ensuremath{h_i(t)}},
  text={\ensuremath{h_i(t)}},
  description={one-to-one mapping from $t$-chronological time to $m$-individual time; note that $h_i(E_i) = 0$ and $h_i(T_i) = M_i$; writing just $h(t)$ denotes a general function which can take a vector of start times}
}

\newglossaryentry{gls_Oi_ds} {
  name={\ensuremath{O^{'}_i(m)}},
  text={\ensuremath{O^{'}_i(m)}},
  description={time $m$-specific p-dimensional variable, where $O^{'}_i(m) = (W^{'}_i(m), Y^{'}_i(m))$ and $O^{'}_i(m) = O_i(h_i(t)) = (W_i(h_i(t)), Y_i(h_i(t)))$; in order to relate $O^{'}_i(m)$ (time-series specific time) to $O_i(h_i(t))$ (chronological time), we need the current chronological time $t$ and the subject's entry time, $E_i$}
}

\newglossaryentry{gls_Oi_h} {
  name={\ensuremath{O_i(h_i(t))}},
  text={\ensuremath{O_i(h_i(t))}},
  description={chronological time $t$-specific p-dimensional variable, where $O_i(h_i(t)) = O^{'}_i(m) = (W_i(h_i(t)), Y_i(h_i(t)))$ and $h_i(t) = t - E_i$; in order to relate $O_i(h_i(t))$ (chronological time) to $O^{'}_i(m)$ (time-series specific time), we need the current chronological time $t$ and the subject's entry time, $E_i$}
}

\newglossaryentry{gls_nt} {
  name={\ensuremath{n(t)}},
  text={\ensuremath{n(t)}},
  description={total number of subjects in the study at chronological time $t$}
}

\newglossaryentry{gls_nmt} {
  name={\ensuremath{n_m(t)}},
  text={\ensuremath{n_m(t)}},
  description={total number of subjects in the study with $m$ points by chronological time $t$}
}

\newglossaryentry{gls_Fmt} {
  name={\ensuremath{F^{n(t)}(t)}},
  text={\ensuremath{F^{n(t)}(t)}},
  description={collection of $n(t)$ observed time-series enrolled at or before time point $t$; we write $F^{n(t)}(t) \equiv \{O_i(h_i(t)): \forall i \text{ where }E_i \leq t\}$}
}

\newglossaryentry{gls_Fbar} {
  name={\ensuremath{\overline{F}(t-1)}},
  text={\ensuremath{\overline{F}(t-1)}},
  description={time $t$-specific history of the available series with start time before chronological time $t$, where $\overline{F}(t-1) = \overline{O}(h(t-1)) = (F(0), \ldots, F(t-1))$; $\overline{F}_i(t-1)$ denotes the sample $i$ time $t$-specific history with start time before chronological time $t$}
}

\newglossaryentry{gls_Ch} {
  name={\ensuremath{C_h(i,s,E_i,T_i)}},
  text={\ensuremath{C_h(i,s,E_i,T_i)}},
  description={time $h_i(s)$- and unit $i$-specific record where $C_h(i,s,E_i,T_i) = (X_i, Z_i(h_i(s-1)), Y_i(h(s)),E_i,T_i)$}
} 

\newglossaryentry{gls_I} {
  name={\ensuremath{\mathcal{I}}},
  text={\ensuremath{\mathcal{I}}},
  description={set of all samples $i$ with start date before current chronological time $t$ $(E_i \leq t)$ with data still being collected $(t \leq T_i)$}
} 

\newglossaryentry{gls_risk_m} {
  name={\ensuremath{R_m(P_{0}, \psi)}},
  text={\ensuremath{R_m(P_{0}, \psi)}},
  description={true risk of $\psi$ for a $m$-time-point-specific prediction, defined as the sum over time and available samples of the expected value of the loss with respect to $P_{0}^n$; 
  $R_m(P_{0}, \psi) = \sum_{t=1}^{\tau} \sum_{i \in \mathcal{I}}  \mathbb{I}(h_i(t) = m) E_{P_{0,O_i}} [L(\psi)(C_h(i,t,E_i,T_i)) |X_i, Z_i(h_i(t-1))] $
  }
  }

\newglossaryentry{gls_risk_cv_m} {
  name={\ensuremath{R_{CV,m}(P_{n,t}^1, \hat{\Psi}_k(\cdot))}},
  text={\ensuremath{R_{CV,m}(P_{n,t}^1, \hat{\Psi}_k(\cdot))}},
  description={online cross-validated risk for candidate estimator $k$ defined as an empirical average of the loss with respect to $P_{n,t}^1$ at individual time $m$}
  } 
  
\newglossaryentry{gls_kntm} {
  name={\ensuremath{k_{n,t,m}}},
  text={\ensuremath{k_{n,t,m}}},
  description={learner that minimizes the online cross-validated risk for individual time $m$, the $m$-discrete online cross-validation selector
  }
}  

\newglossaryentry{gls_alpha_ntm} {
  name={\ensuremath{\alpha_{n,t,m}}},
  text={\ensuremath{\alpha_{n,t,m}}},
  description={weight for the ensemble of candidate estimators $\hat{\Psi}_k$ based on $P_{n,t}$ for individual time $m$ that minimizes the online cross-validated risk}
} 


